Dual Manifold Adversarial Robustness: Defense against Lp and non-Lp Adversarial Attacks

Adversarial training is a popular defense strategy against attack threat models with bounded Lp norms. However, it often degrades the model performance on normal images and the defense does not generalize well to novel attacks. Given the success of deep generative models such as GANs and VAEs in characterizing the underlying manifold of images, we investigate whether or not the aforementioned problems can be remedied by exploiting the underlying manifold information. To this end, we construct an "On-Manifold ImageNet" (OM-ImageNet) dataset by projecting the ImageNet samples onto the manifold learned by StyleGSN. For this dataset, the underlying manifold information is exact. Using OM-ImageNet, we first show that adversarial training in the latent space of images improves both standard accuracy and robustness to on-manifold attacks. However, since no out-of-manifold perturbations are realized, the defense can be broken by Lp adversarial attacks. We further propose Dual Manifold Adversarial Training (DMAT) where adversarial perturbations in both latent and image spaces are used in robustifying the model. Our DMAT improves performance on normal images, and achieves comparable robustness to the standard adversarial training against Lp attacks. In addition, we observe that models defended by DMAT achieve improved robustness against novel attacks which manipulate images by global color shifts or various types of image filtering. Interestingly, similar improvements are also achieved when the defended models are tested on out-of-manifold natural images. These results demonstrate the potential benefits of using manifold information in enhancing robustness of deep learning models against various types of novel adversarial attacks.

==> figures/AT_comparison_orig.tex <==
\begin{figure*}[t!]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}[t]{0.25\textwidth}
        \raisebox{-12ex}{\rotatebox[origin=c]{90}{\text{Fog}}}
    \end{subfigure}
    \hspace{-3cm}
    \begin{subfigure}[t]{0.25\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{png/AT_comparison/original/image_005.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_sgd/image_adv_005.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_sgd/image_diff_005.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_normal_adv_pgd5_sgd/image_adv_005.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_normal_adv_pgd5_sgd/image_diff_005.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_fgsm_sgd/image_adv_005.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_fgsm_sgd/image_diff_005.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_pgd5_sgd/image_adv_005.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_pgd5_sgd/image_diff_005.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_pgd5_pgd5_sgd/image_adv_005.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_pgd5_pgd5_sgd/image_diff_005.png}}
    \end{subfigure}
    \\
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}[t]{0.25\textwidth}
        \raisebox{-12ex}{\rotatebox[origin=c]{90}{\text{L2}}}
    \end{subfigure}
    \hspace{-3cm}
    \begin{subfigure}[t]{0.25\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{png/AT_comparison/original/image_018.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_sgd/image_adv_018.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_sgd/image_diff_018.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_normal_adv_pgd5_sgd/image_adv_018.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_normal_adv_pgd5_sgd/image_diff_018.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_fgsm_sgd/image_adv_018.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_fgsm_sgd/image_diff_018.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_pgd5_sgd/image_adv_018.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_pgd5_sgd/image_diff_018.png}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_pgd5_pgd5_sgd/image_adv_018.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_pgd5_pgd5_sgd/image_diff_018.png}}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.25\textwidth}
        \raisebox{-12ex}{\rotatebox[origin=c]{90}{\text{JPEG}}}
    \end{subfigure}
    \hspace{-3cm}
    \begin{subfigure}[t]{0.25\textwidth}
        \raisebox{-\height}{\includegraphics[width=\textwidth]{png/AT_comparison/original/image_022.png}}
        \caption*{Original}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_sgd/image_adv_022.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_sgd/image_diff_022.png}}
        \caption*{\stackanchor{Normal}{Training}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_normal_adv_pgd5_sgd/image_adv_022.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_normal_adv_pgd5_sgd/image_diff_022.png}}
        \caption*{\stackanchor{AT}{[PGD-5]}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_fgsm_sgd/image_adv_022.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_fgsm_sgd/image_diff_022.png}}
        \caption*{\stackanchor{OM-AT}{[OM-FGSM]}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_pgd5_sgd/image_adv_022.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_manifold_pgd5_sgd/image_diff_022.png}}
        \caption*{\stackanchor{OM-AT}{[OM-PGD-5]}}
    \end{subfigure}
    \begin{subfigure}[t]{0.125\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_pgd5_pgd5_sgd/image_adv_022.png}}\\
        \raisebox{-\height}{\includegraphics[width=0.99\textwidth]{png/AT_comparison/mixed10_pgd5_pgd5_sgd/image_diff_022.png}}
        \caption*{DMAT}
    \end{subfigure}
    \caption{Visual comparison between adversarial training methods when the adversarial examples are crafted using natural (out-of-manifold) images. Brighter colors indicate larger absolute differences. We can observe that the classifier trained with DMAT is more robust and needs stronger distortions to break.} \label{fig:at_comparison_orig}
\end{figure*}

==> figures/Lp_attack.tex <==






\begin{figure*}[t] 
\centering
\begin{tikzpicture}
\begin{groupplot}[
group style={group size=3 by 1},
width=0.38\textwidth,
ymin=0,ymax=100,
xmin=0,xmax=20,
xlabel={Epoch},
ytick = {0, 25, 50, 75, 100}
]

\nextgroupplot [title={Standard Accuracy},
style={line width=1.0pt},
grid=both,
grid style={line width=.1pt, draw=gray!40},
ylabel=Accuracy,
y label style={at={(axis description cs:-0.1,.5)},anchor=south}]

\addplot[black] table[x=Epoch, y=Normal, col sep=comma,] {clean_acc.csv}; \label{normal}
\addplot[red, mark=+, mark size=1.5pt] table[x=Epoch, y=PGD5_sgd, col sep=comma,] {clean_acc.csv};\label{image_sgd}
\addplot[blue, mark=+, mark size=1.5pt] table[x=Epoch, y=TRADES, col sep=comma,] {clean_acc.csv};\label{trades}

\addplot[green, mark=diamond*, mark size=1.5pt] table[x=Epoch, y=OM-FGSM, col sep=comma,] {clean_acc.csv};\label{latent_fgsm}
\addplot[purple, mark=diamond*, mark size=1.5pt] table[x=Epoch, y=OM-PGD, col sep=comma,] {clean_acc.csv};\label{latent_pgd}
\coordinate (top) at (rel axis cs:0,1);

\nextgroupplot[title={Accuracy on PGD-50},
style={line width=1.0pt},
grid=both,
grid style={line width=.1pt, draw=gray!40}
]
\addplot[black] table[x=Epoch, y=Normal, col sep=comma,] {adv_acc.csv};
\addplot[red, mark=+, mark size=1.5pt] table[x=Epoch, y=PGD5_sgd, col sep=comma,] {adv_acc.csv}; 
\addplot[blue, mark=+, mark size=1.5pt] table[x=Epoch, y=TRADES, col sep=comma,] {adv_acc.csv}; 
\addplot[green, mark=diamond*, mark size=1.5pt] table[x=Epoch, y=OM-FGSM, col sep=comma,] {adv_acc.csv}; 
\addplot[purple, mark=diamond*, mark size=1.5pt] table[x=Epoch, y=OM-PGD, col sep=comma,] {adv_acc.csv};

\nextgroupplot[title={Accuracy on OM-PGD-50},
style={line width=1.0pt},
grid=both,
grid style={line width=.1pt, draw=gray!40}
]
\addplot[black] table[x=Epoch, y=Normal, col sep=comma,] {om_adv_acc.csv};
\addplot[red, mark=+, mark size=1.5pt] table[x=Epoch, y=PGD5_sgd, col sep=comma,] {om_adv_acc.csv}; 
\addplot[blue, mark=+, mark size=1.5pt] table[x=Epoch, y=TRADES, col sep=comma,] {om_adv_acc.csv}; 
\addplot[green, mark=diamond*, mark size=1.5pt] table[x=Epoch, y=OM-FGSM, col sep=comma,] {om_adv_acc.csv}; 
\addplot[purple, mark=diamond*, mark size=1.5pt] table[x=Epoch, y=OM-PGD, col sep=comma,] {om_adv_acc.csv};

\coordinate (bot) at (rel axis cs:1,0);
\end{groupplot}
% legend
  \path (top|-current bounding box.south)--
        coordinate(legendpos)
        (bot|-current bounding box.south);
  \matrix[
      matrix of nodes,
      anchor=north,
      draw,
      inner sep=0.2em,
    ]at([yshift=-1ex]legendpos)
    { \ref{normal}& Normal&[5pt]
      \ref{image_sgd}& AT [PGD-5] &[5pt]
      \ref{trades}& TRADES [PGD-5] &[5pt] \\
      \ref{latent_fgsm}& OM-AT [OM-FGSM] &[5pt]
      \ref{latent_pgd}& OM-AT [OM-PGD-5] &[5pt]\\};
\end{tikzpicture}
\caption{On-manifold adversarial training does not provide robustness to standard attacks. Standard adversarial training does not provide robustness to on-manifold attacks. Left: standard accuracy. Middle: classification accuracy when the trained models are attacked by PGD-50. Right: classification accuracy when the trained models are attacked by OM-PGD-50.}
\label{fig:on_off_AT}
\end{figure*}

==> figures/demo.tex <==

%


\begin{tikzpicture}
\begin{groupplot}[
group style={group size=2 by 2},
width=0.4\textwidth,
xtick=data,
]
\nextgroupplot[title=Turbidez]
\addplot table[x=Dosagem SA, y=Remocao T, col sep=comma,] {dose_sulfato.csv};
\nextgroupplot[title=Cor Aparente]
\addplot table[x=Dosagem SA, y=Remocao C, col sep=comma,] {dose_sulfato.csv};
\nextgroupplot
\addplot[red, mark=*] table[x=Dosagem Q, y=Remocao T, col sep=comma,] {dose_quitosana.csv};
\nextgroupplot
\addplot[red, mark=*] table[x=Dosagem Q, y=Remocao C, col sep=comma,] {dose_quitosana.csv};    
\end{groupplot}
\node[anchor=north] (title-x) at ($(group c1r2.south east)!0.5!(group c2r2.south west)-(0,0.5cm)$) {Dosagem de Coagulante $(mg/L)$};
\node[anchor=south, rotate=90] (title-y) at ($(group c1r1.south west)!0.5!(group c1r2.north west)-(0.85,0cm)$) {Remoção (\%)};
\end{tikzpicture}

==> figures/demo2.tex <==


\begin{tikzpicture}
\begin{groupplot}[
group style={group size=3 by 1},
width=0.4\textwidth,
xtick=data,
]
\nextgroupplot
\addplot[blue, mark=*] table[x=Epoch, y=Image, col sep=comma,] {clean_acc.csv}; \label{image}
\addplot[black] table[x=Epoch, y=Dual, col sep=comma,] {clean_acc.csv};
\coordinate (top) at (rel axis cs:0,1);
\nextgroupplot
\addplot[blue, mark=*] table[x=Epoch, y=Image, col sep=comma,] {clean_acc.csv};
\addplot[red] table[x=Epoch, y=Latent, col sep=comma,] {clean_acc.csv}; \label{latent}
\nextgroupplot
\addplot[red] table[x=Epoch, y=Latent, col sep=comma,] {clean_acc.csv};
\addplot[black] table[x=Epoch, y=Dual, col sep=comma,] {clean_acc.csv}; \label{dual}
\coordinate (bot) at (rel axis cs:1,0);
\end{groupplot}
% legend
  \path (top|-current bounding box.south)--
        coordinate(legendpos)
        (bot|-current bounding box.south);
  \matrix[
      matrix of nodes,
      anchor=north,
      draw,
      inner sep=0.2em,
    ]at([yshift=-1ex]legendpos)
    { \ref{image}& Image&[5pt]
      \ref{latent}& Latent&[5pt]
      \ref{dual}& Dual&[5pt]\\};
\end{tikzpicture}

==> figures/learning_rate.tex <==


\begin{figure*}[t] 
\centering
\begin{tikzpicture}
\begin{groupplot}[
group style={group size=1 by 1},
width=0.38\textwidth,
ymin=0,ymax=0.5,
xmin=0,xmax=20,
xlabel={Epoch}
]

\nextgroupplot [title={},
style={line width=1.0pt},
grid=both,
grid style={line width=.1pt, draw=gray!40},
ylabel=Learning Rate,
y label style={at={(axis description cs:-0.15,.5)},anchor=south}]

\addplot[blue] table[x=Epoch, y=LR, col sep=comma,] {lr.csv}; 
\end{groupplot}
\end{tikzpicture}
\caption{Learning rate scheduling during training.}
\label{fig:lr}
\end{figure*}

==> figures/perceptual_comparison.tex <==
\begin{figure*}[t]
  \centering
%   \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{12cm}{0cm}}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/original/image_000.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/elastic/image_adv_000.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/fog/image_adv_000.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/jpeg/image_adv_000.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/snow/image_adv_000.png}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/original/image_020.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/elastic/image_adv_020.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/fog/image_adv_020.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/jpeg/image_adv_020.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/snow/image_adv_020.png}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/original/image_006.png}
  \caption{Original}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/elastic/image_adv_006.png}
  \caption{Elastic}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/fog/image_adv_006.png}
  \caption{Fog}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/jpeg/image_adv_006.png}
  \caption{JPEG compression}
  \end{subfigure}
  \begin{subfigure}[t]{0.19\textwidth}
  \includegraphics[width=\textwidth]{png/Perceptual_comparison/snow/image_adv_006.png}
  \caption{Snow}
  \end{subfigure}
  \caption{Sample adversarial images from different perceptual adversarial attacks. } \label{fig:perceptual_comparison}
\end{figure*}

==> figures/projection.tex <==
\begin{figure*}[t!]
  \centering
%   \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{12cm}{0cm}}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_000.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_000.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_001.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_001.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_002.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_002.png}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_003.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_003.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_004.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_004.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_005.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_005.png}
  \end{subfigure}
  \\
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_006.png}
  \caption*{Original}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_006.png}
  \caption*{\stackanchor{Projected}{(On-manifold)}}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_007.png}
  \caption*{Original}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_007.png}
  \caption*{\stackanchor{Projected}{(On-manifold)}}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/orig/image_008.png}
  \caption*{Original}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\textwidth}
  \includegraphics[width=\textwidth]{png/projection/image_008.png}
  \caption*{\stackanchor{Projected}{(On-manifold)}}
  \end{subfigure}
  \caption{Visual comparison between original images and projected images. Even though some fine-grained details are lost after projection, the diversity of the projected images is still high. More importantly, the manifold information for these projected images is \emph{exact}.} \label{fig:projection}
\end{figure*}

==> tables/seen_attacks_param.tex <==
\begin{table*}[h!]
\caption{Parameter settings for standard and on-manifold attack threat models.}
\label{table:seen_attacks_param}
\centering
\small
\begin{tabular}{ccccc}
\toprule
  PGD-5  &  PGD-50 & OM-FGSM & OM-PGD-5 & OM-PGD-50 \\
  \midrule
  $\epsilon = 4/255$  &  $\epsilon = 4/255$ & $\eta = 0.02$  & $\eta = 0.02$  & $\eta = 0.02$ \\
  $\epsilon_{iter} = 1/255$  & $\epsilon_{iter} = 1/255$  & $\eta_{iter} = 0.005$  & $\eta_{iter} = 0.005$  & $\eta_{iter} = 0.005$ \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/unseen_attacks_ablation.tex <==
\begin{table*}[h!]
\caption{Classification accuracy against unseen attacks applied to OM-ImageNet test set.} \label{table:unseen_attacks_ablation}
\centering
\small
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
                & Standard  &  Fog     &  Snow    &  Elastic   &   Gabor   &  JPEG &  $L_2$ \\
\midrule
$\epsilon=4/255, \epsilon_{iter}=1/255$  & 77.96\% & 31.78\% & 51.19\%  &  56.09\%   &  51.61\%   & 14.31\%   & 51.36\% \\
$\epsilon=2/255, \epsilon_{iter}=0.5/255$  & 79.29\% & 31.91\% & 43.45\%  & 52.82\% & 39.15\% & 5.84\% & 43.67\% \\
$\epsilon=1/255, \epsilon_{iter}=0.25/255$ & 79.84\% & 29.20\% & 35.35\%  & 49.51\% & 24.35\% & 2.71\% & 32.28\% \\
\midrule
$\eta = 0.02, \eta_{iter}=0.005$ & 77.96\% & 31.78\% & 51.19\%  &  56.09\%   &  51.61\%   & 14.31\%   & 51.36\% \\
$\eta = 0.01, \eta_{iter}=0.004$ & 77.34\% & 26.35\% & 49.49\% &  54.07\% &  51.63\%  &  13.22\% & 47.81\% \\
$\eta = 0.005, \eta_{iter}=0.002$ & 76.24\% & 22.40\% & 46.17\% & 51.28\%  &  50.00\% &  13.79\% & 43.85\% \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/unseen_attacks_param.tex <==
\begin{table*}[h!]
\caption{Parameter settings for the novel attacks.}
\label{table:unseen_attacks_param}
\centering
\small
\begin{tabular}{lcccccc}
\toprule
  & Fog    &    Snow    & Elastic    &    Gabor   &     JPEG   &     $L_2$ \\
\midrule
$\epsilon$  & 128    &    0.062  & 0.500        &     12.500   &   1024     &   1200 \\
Step Size   & 0.002 & 0.002 & 0.035 & 0.002 & 72.407 & 170 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/unseen_attacks_trades.tex <==
\begin{table*}[h!]
\caption{Classification accuracy against known (PGD-50 and OM-PGD-50) and unseen attacks applied to OM-ImageNet test set. Even for TRADES, the benefit of using manifold information can also be observed.} \label{table:unseen_attacks_trades}
\centering
\small
\begin{tabular}{@{}lrr|rrrrrr@{}}
\toprule
Method          &    PGD-50  &  \stackanchor{OM-}{PGD-50}    &  Fog     &  Snow    &  Elastic   &   Gabor   &  JPEG &  $L_2$ \\
\midrule
Normal Training    &   0.00\%  &  0.26\% &  0.03\%   &  0.06\%  &  1.20\%    &   0.03\%  &  0.00\%  & 1.70\%  \\
AT [PGD-5]      &  \textbf{38.88\%}   &  7.23\% &  19.76\%  & 46.39\%  &  50.32\%   &  50.43\%  & 10.23\%  & 41.98\% \\
OM-AT [OM-FGSM]  & 0.03\%   &  20.19\%    & 11.12\% & 13.82\%  &  34.07\%   &  1.50\%   & 0.26\%   & 2.27\%  \\
OM-AT [OM-PGD-5]  & 0.25\%  &  \textbf{27.53\%}    & 22.39\% & 28.38\%  &  48.74\%   &  5.19\%    & 0.49\%   & 5.92\%  \\
DMAT              & 37.86\%  &  20.53\%    & \textbf{31.78\%} & \textbf{51.19\%}  &  \textbf{56.09\%}   &  \textbf{51.61\%}   & \textbf{14.31\%}   & \textbf{51.36\%}  \\
\midrule
TRADES        & \textbf{46.06\%}  &  8.92\%    & 18.14\% & \textbf{47.63\%} & 53.32\% & \textbf{54.33\%} & 14.06\% & 46.36\% \\
DMAT + TRADES & 42.57\%  &  \textbf{26.82\%}   & \textbf{30.64\%} & 46.62\% & \textbf{56.38\%} & 53.43\% & \textbf{23.62\%} & \textbf{55.09\%} \\
\bottomrule
\end{tabular}
\end{table*}
